Focus-style proof systems and interpolation for the alternation-free $\mu$-calculus

In this paper we introduce a cut-free sequent calculus for the alternation-free fragment of the modal $\mu$-calculus. This system allows for cyclic proofs and uses a simple focus mechanism to control the unravelling of fixpoints along infinite branches. We show that the proof system is sound and complete and apply it to prove that the alternation-free fragment has the Craig interpolation property.

==> sec-extra.tex <==
\section{Additional proofs}

\newcommand{\depth}[1]{|{#1}|_d}

\begin{definition}
 An annotated sequent $\Sigma$ is \emph{thin} if there is no formula
$\varphi \in \AFMC$ such that $\varphi^f \in \Sigma$ and $\varphi^u \in
\Sigma$.
 A pre-proof $\Pi = (T,P,\Si,\pLab)$ is \emph{thin} if for all $v \in T$
with $\varphi^f,\varphi^u \in \Si_v$ we have that $\pLab_v =
\RuWeak$ and $\varphi^u \notin \Si_u$ for the unique $u$ with $P v
u$.\footnote{It might be worth considering the weaker condition that
$\varphi^u$ is not a side formula of the rule application.}
\end{definition}

\begin{definition}
 A pre-proof $\Pi = (T,P,\Si,\pLab)$ of $\Gamma$ with open assumptions
$\Delta_1,\dots,\Delta_n$ is \emph{non-circular} if
\begin{enumerate}
 \item $\Pi$ is finite, and
 \item the discharge rule is not applied in $\Pi$.
\end{enumerate}
\end{definition}

\begin{definition}
 The \emph{depth} of a non-circular pre-proof $\Pi = (T,P,\Si,\pLab)$ is
maximal number of applications of rules other than the weakening rule on
branch of $\Pi$.
\end{definition}

\begin{definition}
 Let $\Sigma$ and $\Gamma$ be annotated sequents. We define
$\morefocus{\Sigma}{\Gamma}$ to hold if
\begin{enumerate}
 \item $\uls{\Sigma} = \uls{\Gamma}$, and
 \item $\varphi^f \in \Sigma$ implies $\varphi^f \in \Gamma$.
\end{enumerate}
\end{definition}

\begin{definition}
 A non-circular pre-proof $\Pi'$ of $\Gamma'$ is a \emph{focus
simulation} of a pre-proof $\Pi$ of $\Gamma$ if
\begin{enumerate}
 \item $\morefocus{\Gamma}{\Gamma'}$,
 \item for every open assumption $\Delta'$ of $\Pi'$ there is an open
assumption $\Delta$ of $\Pi$ such that $\morefocus{\Delta}{\Delta'}$.
 \item $\depth{\Pi'} \leq \depth{\Pi}$.
\end{enumerate}
\end{definition}

\begin{definition}
 An application of a boolean or fixpoint rule in a pre-proof $\Pi =
(T,P,\Si,\pLab)$ is \emph{destructive} if the principal formula does not
occur in the sequent at any of the premises of the application. More
precisely, an application of a rule at a node $v$ is \emph{destructive}
if for the principal formula $\varphi^a \in \Si_v$ it holds that
$\varphi^a \notin \Si_u$ for all $u$ with $R v u$. The proof $\Pi$ is
\emph{destructive} if all applications of the boolean rules and the
fixpoint rules in $\Pi$ are destructive.
\end{definition}

The main result is:
\begin{theorem}
 Every \Focusinf-derivable sequent $\Sigma$ has a thin and destructive
\Focusinf-proof.
\end{theorem}

To proof this result we introduce some additional notions.

\begin{definition}
 A pre-proof $\Pi = (T,P,\Si,\pLab)$ of $\Gamma$ with open assumptions
$\Delta_1,\dots,\Delta_n$ is \emph{local} if
\begin{enumerate}
 \item $\Pi$ is non-circular (that is, it is finite and does not contain
applications of the discharge rule),
 \item $\Pi$ does not contain applications of the modal rule \RuBox, and
 \item Every assumption $\Delta$ of $\Pi$ only contains modal formulas. 
\end{enumerate}
\end{definition}

\begin{definition}
 Let $\xi^a$ be an annotated formula. The \emph{$\xi^a$-complexity} of a
pre-proof $\Pi = (T,P,\Si,\pLab)$ with root $r$ is the number of nodes
$v$ in $\Pi$ such that $\xi^a \in \Si_u$ for every node $u \in [r,v]$.
\end{definition}

\begin{proposition} \label{p:thin simulation}
 Let $\Pi$ be a non-circular, thin and destructive pre-proof of $\Gamma$
and $\Gamma'$ a sequent such that $\morefocus{\Gamma}{\Gamma'}$. Then
there is a thin and destructive focus simulation $\Pi'$ of $\Pi$ that
proves the sequent $\Gamma'$.
\end{proposition}
\begin{proof}
I hope this can be proved with an induction on the depth of $\Pi$,
moving from the root to the leaves.
\end{proof}

\begin{proposition} \label{p:root}
 Let $\Pi$ be a thin local pre-proof of $\Gamma$ such that all
occurrences of boolean or fixpoint rules, except the one at the root $r$,
are destructive. Then, there is a thin and destructive local pre-proof
$\Pi'$ of $\Gamma$ such that $\Pi'$ is a focus simulation of $\Pi$.
\end{proposition}
\begin{proof}
The proof is a nested induction. The outer induction proves the
statement of the proposition with an induction over the depth of the
local pre-proof $\Pi$.

In the base case we have that $\Pi$ consists of just the root node,
which is either an open assumption or an axiomatic leaf. Trivially,
$\Pi$ is destructive in these cases.

For the inductive step assume that the claim holds for all pre-proofs of
depth that is strictly smaller than the depth of $\Pi$. Note that we
might assume without loss of generality that the rule applied at the
root of $\Pi$ is either a boolean or a fixpoint rule and that this
application is not destructive. In all other cases $\Pi$ is already a
destructive proof, because by assumption all rule applications that are
not at the root are destructive.

The proof proceeds by a case distinction depending on the rule that is
applied at the root $r$ of $\Pi$. In all cases we make use of the
following claim, which we proof further below using an inner induction.
\begin{claimfirst} \label{cl:commuting rules}
 Assume that $\xi$ is a disjunction, a conjunction or a fixpoint
formula.
 Let $\Lambda$ be a destructive, thin and local pre-proof of
$\Gamma^\star$ with $\xi^a \in \Gamma^\star$ and $\depth{\Lambda} <
\depth{\Pi}$. Then, there is a destructive, local and thin pre-proof
$\Lambda'$ of $\Gamma^\star$ such that the $\xi^a$-complexity of
$\Lambda'$ is $1$ and $\Lambda'$ is a focus simulation of $\Lambda$.
\end{claimfirst}
Assuming that we have already established this claim let us consider all
the cases of the outer induction.

\textit{Case $\pLab(r) = \RuOr$:} 
In this case $\Si_r = (\xi_0 \lor \xi_1)^a, \Gamma$ and we have $\Si_v =
\xi_0^a, \xi_1^a, \Gamma$ for the unique child $v$ of $r$. Let $\xi =
\xi_0 \lor \xi_1$. We can restrict to the case where $\xi^a \in \Gamma$,
because otherwise our proof is already destructive. We then apply
Claim~\ref{cl:commuting rules} to the local proof $\Pi_v$ starting at
$v$ to obtain a thin and destructive proof $\Lambda'$ of $\xi_0^a,
\xi_1^a,\xi^a, \Gamma'$, where $\Gamma' = \Gamma \setminus \{\xi^a\}$
such that $\Lambda'$ is a focus simulation of $\Pi_v$ and the
$\xi^a$-complexity of $\Lambda'$ is $1$. The latter means that at the
root $w$ of $\Lambda'$ we either weaken $\xi^a$ away with an application
of \RuWeak or we have a destructive application of \RuOr to $\xi^a$. We
consider both cases separately.

If at $w$ there is an application of weakening that removes $\xi^a$ then
$\Gamma^- \subseteq \xi_0^a, \xi_1^a, \Gamma'$ such that $\Gamma^-$ is
the annotated sequent at the child $u$ of $w$. Let $\Lambda'_u$ be the
proof of $\Gamma^-$ that is rooted at $u$, for which we have that
$\depth{\Lambda'_u} \leq \depth{\Lambda'} \leq \depth{\Pi_v} < \depth{\Pi}$.
We then let $\Pi'$ be the following proof:
\begin{center}
\begin{prooftree}
\AxiomC{$\Lambda'_u$}
\noLine
\UnaryInfC{$\Gamma^-$}
\RightLabel{$\RuWeak$}
\UnaryInfC{$\xi_0^a, \xi_1^a, \Gamma'$}
\RightLabel{$\RuOr$}
\UnaryInfC{$(\xi_0 \lor \xi_1)^a, \Gamma'$}
\end{prooftree}
\end{center}
Clearly, this proof is of a depth bound by $\depth{\Pi}$, it is
destructive because $\xi^a \notin \Gamma'$ and it is a proof of the
right sequent because $\xi^a, \Gamma' = \xi^a,\Gamma$. To see that this
proof is thin observe that because $\Lambda'$ is thin the weakening that
is applied at $w$ removes all duplicated formulas from $\xi_0^a,
\xi_1^a,\xi^a, \Gamma'$ and thus $\Gamma^-$ does not contain any such
duplications. Clearly, this entails that the above weakening in $\Pi'$
removes all duplications that might exist in $\xi_0^a, \xi_1^a,
\Gamma'$.

\texttt{Here, we assume that the weakening rule removes all
duplications at once.}

If at $w$ there is an destructive application of \RuOr to $\xi^a$ then
at the child $u$ of $w$ there is a destructive local pre-proof
$\Lambda'_u$ of
$\xi_0^a, \xi_1^a, \Gamma'$ of a depth that is at least $2$ smaller than
the depth of $\Pi$. We can thus let $\Pi'$ be the following proof:
\begin{center}
\begin{prooftree}
\AxiomC{$\Lambda'_u$}
\noLine
\UnaryInfC{$\xi_0^a, \xi_1^a, \Gamma'$}
\RightLabel{$\RuOr$}
\UnaryInfC{$(\xi_0 \lor \xi_1)^a, \Gamma'$}
\end{prooftree}
\end{center}
This construction preserves thinness because if the sequent $\xi_0^a,\xi_1^a,
\Gamma'$ would contain a formula both focused and unfocused then so
would $\Si_v = \xi_0^a, \xi_1^a, \Gamma$ and thus the rule applied at
$v$ would need to be weakening.

\textit{Case $\pLab(r) = \RuAnd$:} 
In this case we have that $\Si_r = (\xi_0 \land \xi_1)^a, \Gamma$
with principal formula $\xi = \xi_0 \land \xi_1$ and there must be two
children $v_0$ and $v_1$ of $r$ such that the pre-proof $\Pi_{v_i}$ rooted at
$v_i$ proves the sequent $\Si_{v_i} = \xi_i^a, \Gamma$
for $i \in \{0,1\}$. Let $\Gamma' = \Gamma \setminus \{\xi^a\}$. We
show that for both $i \in \{0,1\}$
\begin{equation} \label{eq:proofs for conjuncts}
 \mbox{there is a thin and destructive local pre-proof } \Lambda^-_i
\mbox{ of } \xi_i^a, \Gamma' \mbox{ such that $\Lambda^-_i$ is a thin
simulation of $\Pi_{v_i}$}.
\end{equation}

To prove \eqref{eq:proofs for conjuncts} fix $i \in \{0,1\}$. Then
consider the proof $\Pi_{v_i}$ of $\xi_i^a, \Gamma$ that is rooted at
the child $v_i$ inside of $\Pi$. Clearly, $\depth{\Pi_{v_i}} <
\depth{\Pi}$. Moreover, we can assume that $\xi^a \in \Gamma$ because
otherwise we can just let $\Lambda^-_i = \Pi_{v_i}$.

% HERE

Because of $\xi^a \in \Gamma$ we can apply Claim~\ref{cl:communting
rules} to $\Pi_{v_i}$ to obtain a destructive, local pre-proof
$\Lambda'_i$ of $\xi_i^a, \Gamma = \xi_i^a, \xi^a, \Gamma'$ such that
$\Lambda'_i$ is a thin simulation of $\Pi_{v_i}$ and the
$\xi^a$-complexity of $\Lambda'_i$ is $1$. From the latter it follows
that at the root $w_i$ of $\Lambda'_i$ there must be an application of a
rule that removes the formula $\xi^a$. The only possibilities is that we
either apply $\RuWeak$, weakening $\xi^a$ away or we have a destructive
application of $\RuAnd$ to $\xi^a$.

In the former case we consider the destructive local pre-proof
$\Lambda''_i$ of some subset $\Gamma^- \subseteq \xi_i^a,\Gamma'$ that
is rooted at the unique child of $w_i$ in $\Lambda'_i$. The depth of
$\Lambda''_i$ is strictly smaller than the depth of $\Lambda'_i$ and
thus we can add one application of \RuWeak to $\Lambda''_i$ to obtain
the proof $\Lambda^-_i$ of $\xi_i^a, \Gamma'$ that still has the right
depth as required by \eqref{eq:proofs for conjuncts}. Clearly,
$\Lambda''_i$ will be thin, whenever $\Pi$, and thus $\Pi_i$ and
$\Lambda'_i$, were thin.

In the latter case, where \RuAnd is applied at $w_i$ in $\Lambda'_i$ to
remove $\xi^a$, we have that one of the two children $w_i$
proves the sequent $\xi_i^a,\Gamma'$. The proof that is rooted at this
child inside of $\Lambda'_i$ will be the proof $\Lambda^-_i$ that is
required by \eqref{eq:proofs for conjuncts}. Clearly, it is of strictly
smaller depth than $\Lambda'_i$ and thus $\Pi$, and it is thin whenever
$\Pi$ is thin.

Having established \eqref{eq:proofs for conjuncts} we can now use the
proofs $\Lambda^-_0$ and $\Lambda^-_1$ to construct the required
destructive pre-proof $\Pi$ by just combining the two proofs with a new
destructive application of \RuAnd, as follows:
\begin{center}
\begin{prooftree}
\AxiomC{$\Lambda^-_0$}
\noLine
\UnaryInfC{$\xi_0^a, \Gamma'$}

\AxiomC{$\Lambda^-_1$}
\noLine
\UnaryInfC{$\xi_1^a, \Gamma'$}

\RightLabel{$\RuAnd$}
\BinaryInfC{$(\xi_0 \land \xi_1)^a, \Gamma'$}
\end{prooftree}
\end{center}
This proof is destructive and of the right depth. To see that it is thin
whenever $\Pi$ was thin assume for a contradiction that there is some
formula $\varphi$ such that $\varphi^u,\varphi^f \in (\xi_0 \land
\xi_1)^a, \Gamma'$. This would entail that also $\varphi^u,\varphi^f \in (\xi_0 \land
\xi_1)^a, \Gamma$, which is the sequent at the root $r$ of $\Pi$. But
then it would follow since $\Pi$ is thin that $\pLab(r) = \RuWeak$,
contradicting $\pLab(r) = \RuAnd$.

\textit{Case $\pLab(r) \in \{\RuNu,\RuMu\}$:} 
Let $\pLab(r) = \RuFp{\eta}$. We then have that $\Si_r = \xi^a, \Gamma$
with principal formula $\xi = \eta x . \xi_0$ and $\Si_v = \xi_0[\xi /
x]^{a'}, \Gamma$ for the unique child $v$ of $r$, where $a' = u$ if
$\eta = \nu$ and $a' = a$ if $\eta = \mu$. We can restrict our attention
to the case where $\xi^a \in \Gamma$, because otherwise our proof is
already destructive.

We then apply Claim~\ref{cl:commuting rules} to the local proof starting
at $v$ to obtain a destructive proof $\Lambda'$ of $\xi_0[\xi / x]^{a'},
\xi^a, \Gamma'$, where $\Gamma' = \Gamma \setminus \{\xi^a\}$ such that
$\depth{\Lambda'} < \depth{\Pi}$ and the $\xi^a$-complexity of $\Lambda'$
is $1$. The latter means that at the root $w$ of $\Lambda'$ we either
weaken $\xi^a$ away with an application of \RuWeak or we have a
destructive application of \RuFp{\eta} to $\xi^a$. We consider both
cases separately.

If at $w$ there is an application of weakening that removes $\xi^a$ then
there is a subset $\Gamma^- \subseteq \xi_0[\xi / x]^{a'}, \Gamma'$ and
a destructive local pre-proof $\Lambda^-$ of $\Gamma^-$ with
$\depth{\Lambda^-} < \depth{\Lambda'} < \depth{\Pi}$. We can thus let
$\Pi'$ be the following proof:
\begin{center}
\begin{prooftree}
\AxiomC{$\Lambda^-$}
\noLine
\UnaryInfC{$\Gamma^-$}
\RightLabel{$\RuWeak$}
\UnaryInfC{$\xi_0[\xi / x]^{a'}, \Gamma'$}
\RightLabel{$\RuFp{\eta}$}
\UnaryInfC{$\xi^a, \Gamma'$}
\end{prooftree}
\end{center}
The depth of the proof is not larger than the depth of $\Pi$ and the
proof is destructive because $\xi^a \notin \Gamma'$. For the
preservation of thinness assume that $\Pi$, and thus by
Claim~\ref{cl:commuting rules} $\Lambda'$ and $\Lambda^-$ are thin.
This means that if there is an occurrence of $\varphi^u,\varphi^f \in
\xi_0[\xi / x]^{a'}, \xi^a, \Gamma'$ at the root of $\Lambda'$ then
$\varphi^u \notin \Lambda^-$. Clearly this implies that the weakening in
$\Pi'$ above eliminates any such duplicate occurrence in the annotated
sequent $\xi_0[\xi / x]^{a'}, \Gamma'$

If at $w$ there is an destructive application of \RuFp{\eta} to $\xi^a$
then the child of $w$ is destructive local pre-proof $\Lambda^-$ of
$\xi_0[\xi / x]^{a'}, \Gamma'$ with $\depth{\Lambda^-} <
\depth{\Lambda'} < \depth{\Pi}$. We then define $\Pi'$ to be the
following proof:
\begin{center}
\begin{prooftree}
\AxiomC{$\Lambda^-$}
\noLine
\UnaryInfC{$\xi_0[\xi / x]^{a'}, \Gamma'$}
\RightLabel{$\RuFp{\eta}$}
\UnaryInfC{$\xi^a, \Gamma'$}
\end{prooftree}
\end{center}
Clearly, this is a destructive prove of the right sequent that has a
depth that is bound by the depth of $\Pi$. Moreover, if $\Pi$ and thus
$\Lambda'$ are thin then this proof is thin as well. Any occurrence of
$\varphi^u,\varphi^f \in \xi_0[\xi / x]^{a'}, \Gamma'$ for some
$\varphi$ would entail a similar occurrence $\varphi^u,\varphi^f \in
\xi_0[\xi / x]^{a'}, \Gamma$ at the root $w$ of $\Lambda'$. But would
mean that $\Lambda'$ can not be mean weakening is not applied at $w$.

We have now treated all the cases but still need to supply a proof of
the crucial claim:
\begin{proofof}{Claim~\ref{cl:commuting rules}}
 This claim is proved by an inner induction on the $\xi^a$-complexity of
$\Lambda$. In the base case, where the $\xi^a$-complexity of $\xi$ in
$\Lambda$ is $1$ the claim holds trivially.

In the inductive step assume that the $\xi^a$-complexity of $\Pi$ is $n >
1$. Let $r$ be the root of $\Pi$.

Let us first make an observation about the applicability of the inner
induction hypothesis: For each child $u$ of $r$ we consider the local
pre-proof $\Lambda_u$ of $\Si_u$ that is rooted at $u$ in $\Lambda$.
Because by definition the $\xi^a$-complexity of $\Lambda_u$ is smaller
than the $\xi^a$ complexity of $\Lambda$ the inner inductive hypothesis
applies to $\Lambda_u$. This means that if $\xi^a \in \Si_u$ for some
$a$ then there is a destructive, local pre-proof $\Lambda'_u$ of $\Si_u$
such that the $\xi^a$-complexity of $\Lambda'_u$ is $1$.

To construct the proof $\Lambda'$ we then make a first case distinction
depending on the rule that is applied at the root $r$ of $\Lambda$:

\textit{Case if $r$ is an open leaf or $\pLab(r) \in \{\AxLit,\AxTop\}$:}
These cases are impossible because $\xi^a \in \Si_r$ is a disjunction,
conjunction of fixpoint formula, which is not allowed for nodes that a
local assumption in a local proof or at which an axiom is applied.

\textit{Case $\pLab(r) = \RuOr$:}
In this case $\Si_r = (\varphi_0 \lor \varphi_1)^b,\xi^a,\Gamma'$. Let $u$ be the unique child of $r$.

We can assume that $\xi^a \in \Si_u$ because otherwise the
$\xi^a$-complexity of $\Lambda$ is already $1$. From $\xi^a \in \Si_u$
it follows that $(\varphi_0 \lor \varphi_1)^b \neq \xi^a$ because the
application of \RuOr is destructive. From this it follows that $\Si_u =
\varphi_0^b, \varphi_1^b, \xi^a, \Gamma'$ such that $(\varphi_0 \lor
\varphi_1)^b \notin \Gamma'$. We can then use $\xi^a \in \Si_v$ to apply
the inner induction hypothesis to obtain a destructive, local pre-proof
$\Lambda'_u$ of $\Si_u$ with $\xi^a$-complexity equal to $1$ and
$\depth{\Lambda'_u} \leq \depth{\Lambda_u} < \depth{\Lambda}$.

We make a further case distinction on the rule that is applied at the
root $u'$ of $\Lambda'_u$:

\textit{Subcase if in $\Lambda'_u$ the node $u'$ is an open leaf or the leaf
labeled with an axiom:}
These subcases are impossible because $\xi^a \in \Si_u$ is not of the
right shape.

\textit{Subcase for \RuOr:} It must be that $\xi^a$ is principal formula
of the rule application at the root $u'$ of $\Lambda'_v$ because the
$\xi^a$-complexity of $\Lambda'_u$ is $1$. For the same reason this
application is destructive. Thus, $\xi^a = (\xi_0 \lor \xi_1)^a$ and
$\Lambda'_u$ can be extended to the following proof on the left:
\begin{center}
\begin{minipage}{.45\textwidth}
\begin{prooftree}
\AxiomC{$\vdots$}
\noLine
\UnaryInfC{$\varphi_0^b, \varphi_1^b, \xi_0^a, \xi_1^a, \Gamma'$}
\RightLabel{$\RuOr$}
\UnaryInfC{$\varphi_0^b, \varphi_1^b, (\xi_0 \lor \xi_1)^a, \Gamma'$}
\RightLabel{$\RuOr$}
\UnaryInfC{$(\varphi_0 \lor \varphi_1)^b, (\xi_0 \lor \xi_1)^a, \Gamma'$}
\end{prooftree}
\end{minipage}
% 
\begin{minipage}{.45\textwidth}
\begin{prooftree}
\AxiomC{$\vdots$}
\noLine
\UnaryInfC{$\varphi_0^b, \varphi_1^b, \xi_0^a, \xi_1^a, \Gamma'$}
\RightLabel{$\RuOr$}
\UnaryInfC{$(\varphi_0 \lor \varphi_1)^b, \xi_0^a, \xi_1^a, \Gamma'$}
\RightLabel{$\RuOr$}
\UnaryInfC{$(\varphi_0 \lor \varphi_1)^b, (\xi_0 \lor \xi_1)^a, \Gamma'$}
\end{prooftree}
\end{minipage}
\end{center}
Because the upper application of $\RuOr$ to $\xi^a$ is destructive we
can assume that $\xi^a \notin \Gamma'$.

Let $\Lambda''$ be the proof on the right with root $v''$ and node $u''$
just above the root. Because $\xi^a \neq (\varphi_0 \lor \varphi_1)^b$
and $\xi^a \notin \Gamma'$ it follows that the rule application on the
root $v''$ of $\Lambda''$ is destructive. Moreover, $\Lambda''$ is local
and $\depth{\Lambda''} \leq \depth{\Lambda} < \depth{\Pi}$. Now we would
like to take $\Lambda'$ to be $\Lambda''$. But we can not show that the
upper application of \RuOr at $u''$ is destructive. To fix this issue we
consider the subproof of $\Lambda''$ that is rooted at $u''$ we know
that its depth must be strictly smaller than the depth of $\Lambda''$,
which in turn has a depth that is strictly smaller than the depth of
$\Pi$. We can thus apply the outer inductive hypothesis to the proof
rooted at $u''$ and obtain the desired proof $\Lambda'$.

To see that $\Lambda'$ is thin, whenever $\Lambda$ is thin assume that
$\Lambda$ is thin. Then clearly the sequent $(\varphi_0 \lor
\varphi_1)^b,\xi^a,\Gamma'$ is thin, because it is the sequent at the
root of $\Lambda$ which is thin as the weakening rule is not applied at
$r$ in $\Lambda$.
\texttt{I am not quite sure how to argue, or guarantee, that $(\varphi_0
\lor \varphi)^b, \xi_0^a, \xi_1^a, \Gamma'$ is thin.}

\textit{Subcase for \RuAnd:} 
\begin{center}
\begin{minipage}{.45\textwidth}
\begin{prooftree}
\AxiomC{$\vdots$}
\noLine
\UnaryInfC{$\varphi_0^b, \varphi^b, \xi_0^a, \Gamma'_0$}

\AxiomC{$\vdots$}
\noLine
\UnaryInfC{$\varphi_0^b, \varphi^b, \xi_1^a, \Gamma'_1$}

\RightLabel{$\RuAnd$}
\BinaryInfC{$\varphi_0^b, \varphi_1^b, (\xi_0 \land \xi_1)^a, \Gamma'$}
\RightLabel{$\RuOr$}
\UnaryInfC{$(\varphi_0 \lor \varphi_1)^b, (\xi_0 \land \xi_1)^a, \Gamma'$}
\end{prooftree}
\end{minipage}
% 
\begin{minipage}{.45\textwidth}
\begin{prooftree}
\AxiomC{$\vdots$}
\noLine
\UnaryInfC{$\varphi_0^b, \varphi^b, \xi_0^a, \Gamma'$}
\RightLabel{$\RuOr$}
\UnaryInfC{$(\varphi_0 \lor \varphi_1)^b, \xi_0^a, \Gamma'$}

\AxiomC{$\vdots$}
\noLine
\UnaryInfC{$\varphi_0^b, \varphi^b, \xi_1^a, \Gamma'$}
\RightLabel{$\RuOr$}
\UnaryInfC{$(\varphi_0 \lor \varphi_1)^b, \xi_1^a, \Gamma'$}

\RightLabel{$\RuAnd$}
\BinaryInfC{$(\varphi_0 \lor \varphi_1)^b, (\xi_0 \land \xi_1)^a, \Gamma'$}
\end{prooftree}
\end{minipage}
\end{center}

\textit{Subcase for \RuMu and \RuNu}

\textit{Subcase for \RuWeak:}

\textit{Subcase for \RuFocus:}

\textit{Case $\pLab(r) = \RuAnd$:} 

\textit{Case $\pLab(r) = \RuMu$:} 

\textit{Case $\pLab(r) = \RuNu$:} 

\textit{Case $\pLab(r) = \RuWeak$:} 

\textit{Case $\pLab(r) = \RuFocus$:} 
\end{proofof}
We have now treated all the cases in the proof of
Claim~\ref{cl:communting rules} and have thus proved
Proposition~\ref{p:root}
\end{proof}


==> sec-linear.tex <==
\section{The alternation-free linear $\mu$-calculus}
\label{sec-lin}

\btbs
\item
Note that the alternation-free fragment of the linear $\mu$-calculus is equivalent
to the full version.
\etbs

==> ssec-thinprog.tex <==
\newpage
\subsection{Thin and progressive proofs}

When we prove the soundness of our proof system it will be convenient to work
with (infinite) proofs that are in a certain normal form.
The idea here is that we restrict (as much as possible) attention to sequents
that are \emph{thin} in the sense that they do not feature formulas that are
both in and out of focus, and to proofs that are \emph{progressive} in the sense
that when (from the perspective of proof search) we move from the conclusion of
a boolean or fixpoint rule to its premise(s), we may drop the principal formula.
Theorem~\ref{t:tpp} below states that we can make these assumptions without loss
of generality.

\begin{definition}
 An annotated sequent $\Sigma$ is \emph{thin} if there is no formula
$\phi \in \AFMC$ such that $\phi^f \in \Sigma$ and $\phi^u \in
\Sigma$.
Given an annotated sequent $\Si$, we define its \emph{thinning}
\[
\thin{\Si} \isdef \{ \phi^{f} \mid \phi^{f} \in \Si \} \cup \{ \phi^{u}
\mid \phi^{u} \in \Si, \phi^{f} \not\in \Si \}.
\]
A pre-proof $\Pi = (T,P,\Si,\pLab)$ is \emph{thin} if for all $v \in T$
with $\phi^f,\phi^u \in \Si_v$ we have that $\pLab_v =
\RuWeak$ and $\phi^u \notin \Si_u$ for the unique $u$ with $P v
u$.
\end{definition}

Note that one may obtain the thinning $\thin{\Si}$ from an annotated sequent
$\Si$ by removing the \emph{unfocused} versions of the formulas with a double
occurrence in $\Si$.

The definition of a thin proof implies that whenever a thin
proof contains a sequent that is not thin then this sequent is followed
by applications of the weakening rule until all the duplicate formulas
are weakened away. For example if the sequent $\Sigma_v =
p^u,p^f,q^u,q^f,r$ occurs in a thin proof then at $v$ and all of its
immediate successors there need to be applications of weakening until
only one annotated version of $p$ and one annotated version of $q$ is
left. This might look for instance as follows:
\begin{center}
\begin{prooftree}
\AxiomC{$\vdots$}
\noLine
\UnaryInfC{$p^f,q^u,r$}
\RightLabel{\RuWeak}
\UnaryInfC{$p^f,q^u,q^f,r$}
\RightLabel{\RuWeak}
\UnaryInfC{$p^u,p^f,q^u,q^f,r$}
\noLine
\UnaryInfC{$\vdots$}
\end{prooftree}
\end{center}

% A proof is \emph{progressive} if at any application of a boolean or fixpoint 
% rule, the principal formula does not appear in any of the premises.

\begin{definition}
An application of a boolean or fixpoint rule  at a node $u$ in a pre-proof
$\Pi = (T,P,\Si,\pLab)$ is \emph{progressive} if for the principal formula 
$\phi^a \in \Si_u$ it holds that $\phi^a \notin \Si_v$ for all $v$ with 
$Puv$.\footnote{%
   Note that since we assume guardedness, the principal formula is different
   from its residuals.
   } 
The proof $\Pi$ is \emph{progressive} if all applications of the boolean rules
and the fixpoint rules in $\Pi$ are progressive.
\end{definition}

Our main result is the following.
\begin{theorem}
\label{t:tpp}
Every \Focusinf-derivable sequent $\Phi$ has a thin and progressive
\Focusinf-proof.
\end{theorem}

For the proof of Theorem~\ref{t:tpp} we need some preparations.
Recall that we defined the linear order $\sqsubseteq$ on annotations such that 
$u \sqsubset f$.

\begin{definition}
\label{d:mf}
Let $\Sigma$ and $\Gamma$ be annotated sequents. 
We define $\morefocus{\Gamma}{\Sigma}$ to hold if for all $\phi^a \in \Gamma$
there is a $b \sqsupseteq a$ such that $\phi^b \in \Sigma$.
\end{definition}

\begin{definition} \label{d:backcl}
Let $\Si$ be a set of annotated formulas.
We define $\backcl_0(\Sigma)$ as the set of all annotated formulas $\phi^a$ 
such that either
\begin{enumerate}
\item $\phi^b \in \Sigma$ for some $b \sqsupseteq a$;
\item 
 $\phi = \phi_0 \lor \phi_1$, and $\phi_0^a \in \Sigma$ and $\phi_1^a \in \Sigma$;
\item 
 $\phi = \phi_0 \land \phi_1$, and $\phi_0^a \in \Sigma$ or $\phi_1^a \in \Sigma$;
\item $\phi = \mu x . \phi_0$ and $\phi_0(\phi)^u \in \Sigma$; or 
\item $\phi = \nu x . \phi_0$ and $\phi_0(\phi)^a \in \Sigma$.
\end{enumerate}
%
The map $\backcl_0$ clearly being a monotone operator on the sets of annotated
formulas, we define the \emph{backwards closure} of $\Si$ as the least fixpoint
$\backcl(\Sigma)$ of the operator $\Gamma \mapsto \Sigma \cup 
\backcl_0(\Gamma)$.
\end{definition}

In words, $\backcl(\Sigma)$ is the least set of annotated formulas such that
$\Sigma \subseteq \backcl(\Sigma)$ and $\backcl_0(\backcl(\Sigma)) \subseteq 
\backcl(\Sigma)$. 
The following proposition collects some basic properties of $\backcl$; recall 
that we abbreviate $\allfocus{\Sigma} = \allfocus{\uls{\Si}}$, that is, 
$\allfocus{\Sigma}$ consists of the annotated formulas $\phi^{f}$ such that 
$\phi^a \in \Sigma$ for some $a$. 


\begin{proposition} 
\label{p:progressive facts}\label{p:pf}
The map $\backcl$ is a closure operator over sets of annotated formulas. 
Furthermore, the following hold for any pair of annotated sequents $\Ga,\Si$.
\begin{enumerate}
\item 
If $\morefocus{\Gamma}{\Sigma}$ then $\Gamma \subseteq \backcl(\Sigma)$.
\item 
\label{i:pf:2} 
If $\Gamma \subseteq \backcl(\Sigma)$ and $\Gamma$ contains only atomic or 
modal formulas, then $\morefocus{\Gamma}{\Sigma}$.
\item \label{i:proof rules} 
If $\Gamma$ is the conclusion and $\Sigma$ is one of the premises of an 
application of one of the rules \RuOr, \RuAnd, \RuMu, or \RuNu, then 
$\Gamma \subseteq \backcl(\Sigma)$.
\item \label{i:thinning} 
$\{\phi^u,\phi^f\} \cup \Sigma \subseteq
\backcl(\{\phi^f\} \cup \Sigma)$.
\item \label{i:more focus} 
If $\phi^a \in \backcl(\Sigma)$ for some $a$ then $\phi^u, \phi^f \in 
\backcl(\allfocus{\Sigma})$.
% \item \label{i:some focus} 
% If $\phi^f \in \backcl(\Sigma)$ then $\Sigma$ contains at least one
% formula that is in focus.
\end{enumerate}
\end{proposition}

\begin{proof}
These statements are straightforward consequences of
the Definitions~\ref{d:mf} and~\ref{d:backcl}.

For instance, in order to establish part \eqref{i:more focus} it
suffices to prove the following:
\begin{equation}
\label{eq:974}
\phi^{a} \in \backcl_{0}(\Si) \text{ only if } \phi^{f} \in \backcl(\Si^{f}).
\end{equation}
To see this, take an arbitary annotated formula $\phi^{a} \in \backcl_{0}(\Si)$
and make a case distinction as to the reason why $\phi^{a} \in \backcl_{0}(\Si)$.
(1) If $\phi^b \in \Sigma$ for some $b \sqsupseteq a$, then $\Phi^{f} \in \Si^{f}$,
and so $\phi^{f} \in \backcl_{0}(\Si) \sse \backcl(\Si)$.
(2) If $\phi = \phi_0 \lor \phi_1$, and $\phi_0^a, \phi_1^a \in \Sigma$
then $\phi_0^f, \phi_1^f \in \Si^{f}$, so that $\phi^{f} \in \Si^{f}$.
(3) If $\phi = \phi_0 \land \phi_1$, and $\phi_i^a \in \Sigma$ for some $i \in
\{0,1\}$, then $\phi_i^f \in \Sigma^{f}$ so that $\phi^{f}\in\Si^{f}$.
(4) If $\phi = \mu x . \phi_0$ and $\phi_0(\phi)^u \in \Sigma$, then clearly
also $\phi_0(\phi)^u \in \backcl(\Si)$, and so $\phi^{a} \in 
\backcl(\backcl(\Si)) \sse \backcl(\Si)$.
Finally, (5) if $\phi = \nu x . \phi_0$ and $\phi_0(\phi)^a \in \Sigma$, then
$\phi_0(\phi)^f \in \Si^{f}$, so that $\phi^{f} \in \backcl_{0}(\Si) \sse 
\backcl(\Si)$ indeed.
\end{proof}

% \begin{definition}
% A finite pre-proof $\Pi = (T,P,\Si,\pLab)$ with open assumptions is 
% \emph{non-circular} if it features no applications of the discharge rule, and 
% \emph{local} if in addition it does not contain any application of the rule
% \RuBox.
% \end{definition}
% 
\begin{definition}
A local pre-proof $\Pi'$ of $\Gamma'$ is a \emph{simulation}
of a local pre-proof $\Pi$ of $\Gamma$ if
% \begin{enumerate}
% \item
$\Gamma \subseteq \backcl(\Gamma')$, and
% \item 
for every open assumption $\Delta'$ of $\Pi'$ there is an open assumption 
$\Delta$ of $\Pi$ such that $\Delta \subseteq \backcl(\Delta')$.
% \end{enumerate}
\end{definition}

In the proof below we will frequently use the following proposition, the proof
of which is straightforward.

\begin{proposition} 
	\label{p:thinning}
Let $\Gamma$ and $\Delta$ be two sequents such that $\Gamma \subseteq
\backcl(\Delta)$. 
Then $\thin{\De}$ is thin and satisfies $\Gamma \subseteq \backcl(\thin{\De})$,
and there is a thin, progressive proof $\Pi$ of $\Delta$, which has $\thin{\De}$
as its only open assumption and uses only the weakening rule.
\end{proposition}

\begin{proof}
It is clear that $\thin{\De}$ is thin and that we may write $\De = \{\phi_1^u,
\dots,\phi_n^u\} \cup \thin{\De}$, where $\phi_{1},\ldots,\phi_{n}$ are the 
formulas that occur both focused and unfocused in $\De$. 
We then let $\Pi'$ be the proof that weakens the formulas $\phi_1^u,\dots,
\phi_n^u$ one by one.
By item~\ref{i:thinning} of Proposition~\ref{p:progressive facts} it
follows that $\Delta \subseteq \backcl(\thin{\De})$. 
Thus, $\Gamma
\subseteq \backcl(\Delta)$ implies $\Gamma \subseteq \backcl(\thin{\De})$
because $\backcl$ is a closure operator.
% The amount of detail in the proof is much higher than later on!
\end{proof}

The key technical observation in the proof of Theorem~\ref{t:tpp} is 
Proposition~\ref{p:ps} below.

\begin{definition}
\label{p:baspr}
Recall that a pre-proof $\Pi = (T,P,\Si,\pLab)$ is \emph{basic} if $T$ consists
of the root $r$ and its successors, $\pLab_{r} \neq \RuDischarge{}$ and 
$\pLab_{u} = \star$ for every successor of $r$.
\end{definition}

A basic derivation is thus a pre-proof $\Pi = (T,P,\Si,\pLab)$ of $\Si_{r}$
(where $r$ is the root of $\Pi$) with open assumptions $\{ \Si_{u} \mid u \neq
r \}$.

\begin{proposition} 
\label{p:progressive simulation} \label{p:ps}
Let $\Pi$ be a basic pre-proof of $\Gamma$ and let $\Gamma'$ be a sequent such
that $\Gamma \subseteq \backcl(\Gamma')$. 
Then there is a thin and progressive simulation $\Pi'$ of $\Pi$ that proves the 
sequent $\Gamma'$.
Moreover, if $\pLab_{r} \neq \RuFocus, \RuUnfocus$ then $\Pi'$ does not use
$\RuFocus$ or $\RuUnfocus$, and if $\pLab_{r} = \RuBox$ then $\RuBox$ is
also the rule applied at the root of $\Pi'$.
\end{proposition}

Before we prove this proposition, we first show how our main theorem follows
from it.

\begin{proofof}{Theorem~\ref{t:tpp}}
Let $\Pi = (T,P,\Si,\Ru)$ be a \Focusinf-proof of the sequent $\Phi$, then by
definition we have $\Si_{r} = \Phi^{f}$, where $r$ is the root of $\Pi$.
Obviously we have $\Si_{r} \sse \backcl(\Si_{r})$.

We will transform $\Pi$ into a thin proof of $\Phi$ as follows.
On the basis of Proposition~\ref{p:ps} it is straightforward to define a map 
$\Xi$ which assigns a thin sequent $\Xi_{t}$ to each node $t \in T$, in such
a way that $\Xi_{r} \isdef \Si_{r}$, 
and for every $t \in T$ we find $\Si_{t} \sse \backcl(\Xi_{t})$,
while we also have a thin and progressive pre-proof $\Pi_{t}$ of the sequent 
$\Xi_{t}$ from the assumptions $\{ \Xi_{u} \mid Ptu \}$.
% associated with the successors of $t$.
In addition we know that if $\Ru_{t} \neq \RuFocus, \RuUnfocus$, then the 
derivation $\Pi_{t}$ does not involve the focus rules, and that if $\pLab_{t}
= \RuBox$ then $\RuBox$ is also the rule applied at the root of $\Pi_{t}$.
We obtain a thin and progressive proof $\Pi'$ from this by simply adding all 
these thin and progressive derivations $\Pi_{t}$ to the `skeleton structure'
$(T,P,\Xi)$, in the obvious way.

\rood{
It is easy to show that $\Pi'$ is a pre-proof, and the additional conditions 
on the focus rules and $\RuBox$ guarantee that every infinite branch of $\Pi'$
witnesses infinitely many applicatinos of $\RuBox$, but only finitely
many applications of the focus rules.
To prove the remaining condition on focused formulas, consider an infinite branch
$\al = (v_{n})_{n\in\om}$ of $\Pi'$.
It is easy to see that by construction we may associate an infinite branch 
$\be = (t_{n})_{n\in\om}$ of $\Pi$ with $\al$, together with a map $f: \om \to 
\om$ such that $\Si_{t_{n}} \sse \backcl(\Xi_{v_{f(n)}})$.
This path $\be$ is successful since $\Pi$ is a proof, and so there is a $k \in
\om$ such that for all $n \geq k$ the sequent $\Si_{t_{n}}$ contains a formula
in focus, and $\pLab(t_{n}) \neq \RuFocus$.
But by Proposition~\ref{p:pf}(\ref{i:pf:2}) for any $n\geq k$ such that 
$\pLab(t_{n}) = \RuBox$, the sequent $\Xi_{v_{f(n)}}$ must contain a focused
formula as well.
Since $\al$ features infinitely many applications of $\RuBox$, this implies 
the existence of infinitely many nodes $v_{m}$ on $\al$ such that $\Xi_{v_{m}}$
contains a focused formula.
And since the focus rule is applied only finitely often on $\al$, by 
Proposition~\ref{p:lr1} it follows from this that $\al$ actually contains 
cofinitely many such nodes, as required.
}

Furthermore it is obvious that, being constructed by glueing together thin and
progressive proofs, $\Pi'$ has these properties as well.
Finally, since $\Xi_{r} = \Si_{r} = \Phi^{f}$, we have indeed obtained a proof 
for the plain sequent $\Phi$.
\end{proofof}

\begin{proofof}{Proposition~\ref{p:ps}}
By definition of a basic proof, $\Pi = (T,P,\Si,\Ru)$ consists of nothing more
than a single application of the rule $\Ru \isdef \pLab_{r}$ to the annotated 
sequent $\Gamma = \Si_{r}$, where $r$ is the root of $\Pi$.
Because of Proposition~\ref{p:thinning} we can assume without loss of generality
that $\Gamma'$ is thin. 
We then make a case distinction depending on the rule $\Ru$.

Recall that we use $\RuWeak^*$ to denote a finite (potentially zero) number of 
successive applications of weakening.

\begin{description}

\item[\it Case for \AxLit:]
In this case $\Pi$ is of the form
\begin{center}
\begin{prooftree}
 \AxiomC{\phantom{X}}
 \RightLabel{\AxLit}
 \UnaryInfC{$p^a, \atneg{p}^b$}
\end{prooftree}
\end{center}
The assumption is that $\{p^a,\atneg{p}^b\} \subseteq \backcl(\Gamma')$.
By item~\ref{i:pf:2} in Proposition~\ref{p:progressive facts} it
follows that $p^a,\atneg{p}^b \in \Gamma'$.
We can thus define $\Pi'$ to be the proof
\begin{center}
\begin{prooftree}
 \AxiomC{\phantom{X}}
 \RightLabel{\AxLit}
 \UnaryInfC{$p^a, \atneg{p}^b$}
 \RightLabel{$\RuWeak^*$}
 \UnaryInfC{$\Gamma'$}
\end{prooftree}
\end{center}

\item[\it Case for \AxTop:]
In this case $\Pi$ is of the form
\begin{center}
\begin{prooftree}
 \AxiomC{\phantom{X}}
 \RightLabel{\AxTop}
 \UnaryInfC{$\top^a$}
\end{prooftree}
\end{center}
From the assumption that $\top^a \subseteq \backcl(\Gamma')$ it follows
with item~\ref{i:pf:2} of Proposition~\ref{p:progressive facts}
that that $\top^a \in \Gamma'$. We define $\Pi'$ to be the proof.
\begin{center}
\begin{prooftree}
 \AxiomC{\phantom{X}}
 \RightLabel{\AxLit}
 \UnaryInfC{$\top^a$}
 \RightLabel{$\RuWeak^*$}
 \UnaryInfC{$\Gamma'$}
\end{prooftree}
\end{center}

\item[\it Case for \RuOr:]
In this case $\Gamma = \phi_0 \lor \phi_1,\Sigma$ and $\Pi$ is of
the form
\begin{center}
\begin{prooftree}
 \AxiomC{$\phi_0^a,\phi_1^a,\Sigma$}
 \RightLabel{\RuOr}
 \UnaryInfC{$(\phi_0 \lor \phi_1)^a,\Sigma$}
\end{prooftree}
\end{center}
Let $\phi \isdef \phi_0 \lor \phi_1$. Because $\Gamma \subseteq
\backcl(\Gamma')$ it follows that $\phi^a \in \backcl(\Gamma')$.
By definition of $\backcl$ there are two cases for why this might hold,
either $\phi^b \in \Gamma'$ for $b \sqsupseteq a$ or $\phi_0^a \in
\backcl(\Gamma')$ and $\phi_1 \in \backcl(\Gamma')$.

In the latter case where $\phi_0^a \in \backcl(\Gamma')$ and
$\phi_1 \in \backcl(\Gamma')$ we can let $\Pi'$ consist of just the
sequent $\Gamma'$. This proof is thin and progressive and it clear
follows that $\phi_0^a,\phi_1^a,\Sigma \subseteq \backcl(\Gamma')$
because $\Sigma \subseteq \Gamma \subseteq \backcl(\Gamma')$.

In the former case, where $\phi^b \in \Gamma'$ for some $b
\sqsupseteq a$, consider the proof
\begin{center}
\begin{prooftree}
 \AxiomC{$\phi_0^b,\phi_1^b,\Gamma' \setminus \{\phi^b\}$}
 \RightLabel{\RuOr}
 \UnaryInfC{$(\phi_0 \lor \phi_1)^b,\Gamma' \setminus \{\phi^b\}$}
\end{prooftree}
\end{center}
We let $\Pi'$ be this proof. Clearly, this is a proof of $\Gamma' =
(\phi_0 \lor \phi_1)^b,\Gamma' \setminus \{\phi^b\}$ and it is
progressive. Moreover, we have from the definition of $\backcl$ that
$\phi_0^a,\phi_1^a \subseteq \backcl(\phi_0^b, \phi_1^b)$,
as $b \sqsupseteq a$. By item~\ref{i:proof rules} of
Proposition~\ref{p:progressive facts} it holds that $\Gamma' \subseteq
\backcl(\phi_0^b,\phi_1^b,\Gamma' \setminus \{\phi^b\})$. By
assumption we have that $\Gamma \subseteq \backcl(\Gamma')$ and hence
$\Sigma \subseteq \Gamma \subseteq \backcl(\Gamma') \subseteq
\backcl(\phi_0^b,\phi_1^b,\Gamma' \setminus \{\phi^b\})$.
Putting all of these together it follows that
\[
 \phi_0^a,\phi_1^a,\Sigma \subseteq
\backcl(\phi_0^b,\phi_1^b,\Gamma' \setminus \{\phi^b\}).
\]
It remains to be seen that $\Pi$ can be made thin. For the sequent
$\Gamma'$ at the root of $\Pi$ we have already established that it is
thin. It might be, however, that the open assumption
$\phi_0^b,\phi_1^b,\Gamma' \setminus \{\phi^b\}$ is not thin.
If this is the case we can simply apply Proposition~\ref{p:thinning} and
obtain the required proof.

\item[\it Case for \RuAnd:]
In this case $\Gamma = \phi_0 \land \phi_1,\Sigma$ and $\Pi$ is of
the form
\begin{center}
\begin{prooftree}
 \AxiomC{$\phi_0^a,\Sigma$}
 \AxiomC{$\phi_1^a,\Sigma$}
 \RightLabel{\RuAnd}
 \BinaryInfC{$(\phi_0 \land \phi_1)^a,\Sigma$}
\end{prooftree}
\end{center}
Let $\phi \isdef \phi_0 \land \phi_1$. Because $\Gamma \subseteq
\backcl(\Gamma')$ it follows that $\phi^a \in \backcl(\Gamma')$.
By the definition $\backcl$ we may split into two cases: either $\phi^b \in 
\Gamma'$ for $b \sqsupseteq a$ or $\phi_i^a \in \backcl(\Gamma')$ for some 
$i \in \{0,1\}$.

In the subcase where $\phi_i^a \in \backcl(\Gamma')$ for some $i \in
\{0,1\}$ we let $\Pi'$ just be the sequent $\Gamma'$. This sequent is
thin and the proof is trivially progressive. We need to show that there
is some open assumption $\Delta_i$ of $\Pi$ such that $\Delta_i
\subseteq \backcl(\Gamma')$. Let this be the assumption $\phi_i^a,
\Sigma$. We already know that $\phi_i^a \in \backcl(\Gamma')$, so we
it only remains to be seen that $\Sigma \subseteq \backcl(\Gamma')$. But
this follows because $\Sigma \subseteq \Gamma$ and $\Gamma \subseteq
\backcl(\Gamma')$.

In the other subcase we have that $\phi^b \in \Gamma'$ for some $b
\sqsupseteq a$. We let $\Pi'$ be the proof
\begin{center}
\begin{prooftree}
 \AxiomC{$\phi_0^b,\Gamma' \setminus \{\phi^b\}$}
 \AxiomC{$\phi_1^b,\Gamma' \setminus \{\phi^b\}$}
 \RightLabel{\RuAnd}
 \BinaryInfC{$(\phi_0 \land \phi_1)^b,\Gamma' \setminus
\{\phi^b\}$}
\end{prooftree}
\end{center}
By definition this proof is progressive and it is a proof of $\Gamma' =
(\phi_0 \land \phi_1)^b,\Gamma' \setminus \{\phi^b\}$. We then
show that for each open assumption $\phi_i^b, \Gamma' \setminus
\{\phi^b\}$ of $\Pi$, where $i \in \{0,1\}$, there is the open
assumption $\phi_i^a,\Sigma$ of $\Pi$ such that
\begin{equation*}
 \phi_i^a,\Sigma \subseteq \backcl(\phi_i^b, \Gamma' \setminus
\{\phi^b\}).
\end{equation*}
Because $a \sqsubseteq b$ it is clear that $\phi_i^a \in
\backcl(\{\phi_i^b\})$. So we only need $\Sigma \subseteq
\backcl(\phi_i^b, \Gamma' \setminus \{\phi^b\})$. But this follows
from $\Sigma \subseteq \Gamma \subseteq \backcl(\Gamma')$ and the fact
that $\Gamma' \subseteq \backcl(\phi_i^b,\Gamma' \setminus
\{\phi^b\})$, which is item~\ref{i:proof rules} in
Proposition~\ref{p:progressive facts}. 
Finally, as before, we use Proposition~\ref{p:thinning} to deal with non-thin
open assumptions of $\Pi'$, if any.


\item[\it Case for \RuMu:]
In this case $\Gamma = \mu x . \phi_0(x),\Sigma$ and $\Pi$ is of the
form
\begin{center}
\begin{prooftree}
 \AxiomC{$\phi_0(\phi)^u,\Sigma$}
 \RightLabel{\RuMu}
 \UnaryInfC{$(\mu x . \phi_0(x))^a,\Sigma$}
\end{prooftree}
\end{center}
Here we write $\phi = \mu x . \phi_0(x)$. Because $\Gamma \subseteq
\backcl(\Gamma')$ it follows that $\phi^u \in \backcl(\Gamma')$. 
By definition of $\backcl$ this gives us the cases that either $\phi^b
\in \Gamma'$ for some $b \sqsupseteq a$ or $\phi_0(\phi)^u \in
\backcl(\Gamma')$.

In the subcase where $\phi_0(\phi)^u \in \backcl(\Gamma')$ we let
$\Pi'$ just be the sequent $\Gamma'$. This sequent is thin and the proof
is trivially progressive. We need to show $\phi_0(\phi)^u,\Sigma
\subseteq \backcl(\Gamma')$. Because we are in the subcase for
$\phi_0(\phi)^u \in \backcl(\Gamma')$ it suffice to show that
$\Sigma \subseteq \backcl(\Gamma')$. But this follows because $\Sigma
\subseteq \Gamma$ and $\Gamma \subseteq \backcl(\Gamma')$.

In the other subcase we have that $\phi^b \in \Gamma'$ for some $b
\sqsupseteq a$. We let $\Pi'$ be the proof
\begin{center}
\begin{prooftree}
 \AxiomC{$\phi_0(\phi)^u,\Gamma' \setminus \{\phi^b\}$}
 \RightLabel{\RuMu}
 \UnaryInfC{$(\mu x . \phi_0(x))^b,\Gamma' \setminus
\{\phi^b\}$}
\end{prooftree}
\end{center}
Clearly, this proof is progressive and it is a proof of $\Gamma' =
(\mu x . \phi_0(x))^b,\Gamma' \setminus
\{\phi^b\}$. We can also show that
\[
 \phi_0(\phi)^u,\Sigma \subseteq \backcl(\phi_0(\phi)^u,
\Gamma' \setminus \{\phi^b\}).
\]
For this it clearly suffices to show that $\Sigma \subseteq
\backcl(\phi_0(\phi)^u, \Gamma' \setminus \{\phi^b\})$. This
follows from $\Sigma \subseteq \Gamma \subseteq \backcl(\Gamma')$ and
the fact that $\Gamma' \subseteq \backcl(\phi_0(\phi)^u, \Gamma'
\setminus \{\phi^b\})$, which comes from item~\ref{i:proof rules} in
Proposition~\ref{p:progressive facts}. 
Finally, as before, we use Proposition~\ref{p:thinning} to deal with non-thin
open assumptions of $\Pi'$, if any.


\item[\it Case for \RuNu:]
In this case $\Gamma = \nu x . \phi_0(x),\Sigma$ and $\Pi$ is of the
form
\begin{center}
\begin{prooftree}
 \AxiomC{$\phi_0(\phi)^a,\Sigma$}
 \RightLabel{\RuNu}
 \UnaryInfC{$(\nu x . \phi_0(x))^a,\Sigma$}
\end{prooftree}
\end{center}
Here, we write $\phi = \nu x . \phi_0(x)$. Because $\Gamma \subseteq
\backcl(\Gamma')$ it follows that $\phi^u \in \backcl(\Gamma')$. By
the definition $\backcl$ this gives us the cases that either $\phi^b
\in \Gamma'$ for some $b \sqsupseteq a$ or $\phi_0(\phi)^u \in
\backcl(\Gamma')$.

In the subcase where $\phi_0(\phi)^u \in \backcl(\Gamma')$ we let
$\Pi'$ just be the sequent $\Gamma'$. This sequent is thin and the proof
is trivially progressive. We need to show $\phi_0(\phi)^u,\Sigma
\subseteq \backcl(\Gamma')$. Because we are in the subcase for
$\phi_0(\phi)^u \in \backcl(\Gamma')$ it suffice to show that
$\Sigma \subseteq \backcl(\Gamma')$. But this follows because $\Sigma
\subseteq \Gamma$ and $\Gamma \subseteq \backcl(\Gamma')$.

In the other subcase we have that $\phi^b \in \Gamma'$ for some $b
\sqsupseteq a$. We let $\Pi'$ be the proof
\begin{center}
\begin{prooftree}
 \AxiomC{$\phi_0(\phi)^b,\Gamma' \setminus \{\phi^b\}$}
 \RightLabel{\RuNu}
 \UnaryInfC{$(\nu x . \phi_0(x))^b,\Gamma' \setminus
\{\phi^b\}$}
\end{prooftree}
\end{center}
Clearly, this proof is progressive and it is a proof of $\Gamma' = (\mu
x . \phi_0(x))^b,\Gamma' \setminus \{\phi^b\}$. We can also show
that
\[
 \phi_0(\phi)^a,\Sigma \subseteq \backcl(\phi_0(\phi)^b,
\Gamma' \setminus \{\phi^b\}).
\]
Because $a \sqsubseteq b$ it is clear that $\phi_0(\phi)^a \in
\backcl(\{\phi_0(\phi)^b\})$. So it clearly suffices to show that $\Sigma \subseteq
\backcl(\phi_0(\phi)^b, \Gamma' \setminus \{\phi^b\})$. This
follows from $\Sigma \subseteq \Gamma \subseteq \backcl(\Gamma')$ and
the fact that $\Gamma' \subseteq \backcl(\phi_0(\phi)^b, \Gamma'
\setminus \{\phi^b\})$, which comes from item~\ref{i:proof rules} in
Proposition~\ref{p:progressive facts}. 
Any remaining non-thin open assumptions are dealt with using 
Proposition~\ref{p:thinning}.

\item[\it Case for \RuBox:]
In this case $\Ga$ must be of the form $\Ga = \Box\phi^{a},\dia\Si$, and $\Pi$
is the derivation
\begin{center}
\begin{prooftree}
 \AxiomC{$\phi^{a},\Sigma$}
 \RightLabel{\RuBox}
 \UnaryInfC{$\Box\phi^a,\dia\Sigma$}
\end{prooftree}
\end{center}
Because $\Ga \sse \backcl(\Ga')$ it follows from 
Proposition~\ref{p:pf}\eqref{i:pf:2} that $\morefocus{\Ga}{\Ga'}$.
But then $\Ga'$ must contain a subset of the form $\Box\phi^{b},\dia\Si'$, with 
$a \sqsubseteq b$ and $\morefocus{\Si}{\Si'}$.
%
Consider the following derivation $\Pi'$:
\begin{center}
\begin{prooftree}
 \AxiomC{$\phi^{b},\Sigma'$}
 \RightLabel{\RuBox}
 \UnaryInfC{$\Box\phi^b,\dia\Sigma'$}
\RightLabel{$\RuWeak^*$}
 \UnaryInfC{$\Gamma'$}
\end{prooftree}
\end{center}
It is easy to see that we have $\morefocus{\De}{\De'}$, where $\De \isdef
\phi^{a},\Si$ and $\De' \isdef \phi^{b},\Si'$ are the assumptions of the 
pre-proofs $\Pi$ and $\Pi'$, respectively.
Furthermore, the proof $\Pi'$ is obviously progressive, and if not thin already,
can be made so by applying Proposition~\ref{p:thinning}.

\item[\it Case for \RuWeak:]
In this case $\Gamma = \phi^a,\Sigma$ and $\Pi$ is of the form
\begin{center}
\begin{prooftree}
 \AxiomC{$\Sigma$}
 \RightLabel{\RuWeak}
 \UnaryInfC{$\phi^a,\Sigma$}
\end{prooftree}
\end{center}
We can let $\Pi'$ consist of just the sequent $\Gamma'$. This sequent
is thin and the proof is trivially progressive. We need to show that
$\Sigma \subseteq \backcl(\Gamma')$. Clearly $\Sigma \subseteq \Gamma$,
and $\Gamma \subseteq \backcl(\Gamma')$ holds by assumption.


\item[\it Case for \RuFocus:]
In this case $\Gamma = \phi^a,\Sigma$ and $\Pi$ is of the form
\begin{center}
\begin{prooftree}
 \AxiomC{$\phi^f,\Sigma$}
 \RightLabel{\RuFocus}
 \UnaryInfC{$\phi^u,\Sigma$}
\end{prooftree}
\end{center}
We let $\Pi'$ be the proof
\begin{center}
\begin{prooftree}
 \AxiomC{$\allfocus{(\Gamma')}$}
 \RightLabel{$\RuFocus^*$}
 \UnaryInfC{$\Gamma'$}
\end{prooftree}
\end{center}
Here, $\allfocus{(\Gamma')} = \{\phi^f \mid \phi^a \in \Gamma'
\mbox{ for some } a \in \{u,f\}\}$, as in Proposition~\ref{p:progressive
facts}, and $\RuFocus^*$ are as many applications of the focus rule as
we need to put every formula in $\Gamma'$ in focus. This proof $\Pi'$ is
trivially progressive and it is thin because $\Gamma'$ is thin and hence
changing the annotations of some formulas in $\Gamma'$ in this way still
yields a thin sequent. 
From item~\ref{i:more focus} of
Proposition~\ref{p:progressive facts} it is clear that $\phi^f,\Sigma
\subseteq \backcl{\allfocus{(\Gamma')}}$ is implied by $\phi^u,\Sigma
\subseteq \backcl(\Gamma')$.

\item[\it Case for \RuUnfocus:]
In this case $\Gamma = \phi^f,\Sigma$ and $\Pi$ is of the form
\begin{center}
\begin{prooftree}
 \AxiomC{$\phi^u,\Sigma$}
 \RightLabel{\RuUnfocus}
 \UnaryInfC{$\phi^f,\Sigma$}
\end{prooftree}
\end{center}
We can let $\Pi'$ consist of just the sequent $\Gamma'$. This sequent
is thin and the proof is trivially progressive. We need to show that
$\phi^u,\Sigma \subseteq \backcl(\Gamma')$. By the definition of
$\backcl$ we have that $\phi^u \in \backcl(\phi^f)$. 
Thus $\phi^u, \Sigma \subseteq \backcl(\phi^f,\Sigma)$. 
Moreover, we have by assumption that $\phi^f,\Sigma = \Gamma \subseteq
\backcl(\Gamma')$. 
Putting this together, and using that $\backcl$ is a
closure operator, we get $\phi^u,\Sigma \subseteq \backcl(\Gamma')$.
\end{description}

Since we have covered all the cases in the above case distinction, this proves
the main part of the proposition.
The additional statements about the focus rules and the rule $\RuBox$ can 
easily be verified from the definition of $\Pi'$ given above.
\end{proofof}


